Online Network Utility Maximization: Algorithm, Competitive Analysis, and Applications

We consider an online version of the well-studied network utility maximization problem, where users arrive one by one and an operator makes irrevocable decisions for each user without knowing the details of future arrivals. We propose a threshold-based algorithm and analyze its worst-case performance. We prove that the competitive ratio of the proposed algorithm is linearly increasing in the number of links in a network and show this competitive analysis is tight. Extensive trace-driven simulations are conducted to demonstrate the performance of our proposed algorithm. In addition, since worst-case scenarios rarely occur in practice, we devise an adaptive implementation of our algorithm to improve its average-case performance and validate its effectiveness via simulations.

==> sections/1_introduction.tex <==
% Introduction section

\IEEEPARstart{N}{etwork} utility maximization (NUM) is a well-known optimization paradigm in the networking community. After Kelly initially proposed the framework for understanding rate control in wired networks, there have been a multitude of research works on reverse-engineering network protocols that are originally designed based on engineering intuitions, gaining insights on the reasons for their performance, and guiding a systematic design of future versions of network protocols. The monograph \cite{shakkottai2008network} provides a whole picture of research in this direction. Further more, the framework has been used to model resource allocation in various disciplines ranging from wireless networks to economics, after incorporating related constraints, such as power, quality of service or economic constraints. The utility concept in NUM is originally studied in economics, which models the satisfaction level of a consumer for a good or service. 

In spite of many research activities above, some assumptions made in the existing NUM models still require research attention. In the theory of the basic NUM and its solutions, they usually assumed that the users are static, which yields a more tractable analysis but hurts the applicability of the results. To overcome this, one way is to consider stochastic network dynamics, by assuming that the parameters of NUM are stochastically varying. Stochastic network theory is thus connected with this variant
